Towards a Flexible Scale-out Framework for Efficient Visual Data Query Processing

There is growing interest in visual data management systems that support queries with specialized operations ranging from resizing an image to running complex machine learning models. With a plethora of such operations, the basic need to receive query responses in minimal time takes a hit, especially when the client desires to run multiple such operations in a single query. Existing systems provide an ad-hoc approach where different solutions are clubbed together to provide an end-to-end visual data management system. Unlike such solutions, the Visual Data Management System (VDMS) natively executes queries with multiple operations, thus providing an end-to-end solution. However, a fixed subset of native operations and a synchronous threading architecture limit its generality and scalability. In this paper, we develop VDMS-Async that adds the capability to run user-defined operations with VDMS and execute operations within a query on a remote server. VDMS-Async utilizes an event-driven architecture to create an efficient pipeline for executing operations within a query. Our experiments have shown that VDMS-Async reduces the query execution time by 2-3X compared to existing state-of-the-art systems. Further, remote operations coupled with an event-driven architecture enables VDMS-Async to scale query execution time linearly with the addition of every new remote server. We demonstrate a 64X reduction in query execution time when adding 64 remote servers.

==> Discussion.tex <==
\section{Discussion}\label{discussion}
In this paper, we have shown the effectiveness of \our in performing visual data management involving queries that require simple as well as compute-intensive operations in lower time when compared to the existing solutions. There do exist some key directions that need further analysis to improve \our.

\subsection{Further optimization of CPU Utilization}
As we observed in Section~\ref{evaluation}, when working with a large number of parallel clients, \our does not gain much on the CPU utilization front, and the utilization tends to move towards $100\%$. This limitation restricts \our to work with a larger dataset when performing compute-intensive workloads. We can address this issue by tweaking the event-driven architecture to optimize CPU utilization or running a distributed version of \our that works with a single data store.

\subsection{Better video management}
Currently \our works with videos by extracting frames and performing the operations on these frames. Although this is a norm in visual data management, it also results in higher resource usage. Developing an efficient strategy to manage videos without extracting all frames would improve the overall working and user experience with \our.

\subsection{Intelligent Offloading}
The scaling-out set-up discussed in this paper is a proof-of-concept to highlight another utility of \our's event-driven asynchronous architecture. However, we plan to further improve the set-up such that \our can intelligently decide when to offload the tasks to a remote server and to what number of remote servers based on the workload and the available resources on the remote servers.

==> ScaleOut.tex <==
\section{Scaling out VDMS}\label{scaleout}

\begin{itemize}
    \item Why scaleout
    \item Scaleout design
\end{itemize}
